Demon in the Variant: Statistical Analysis of DNNs for Robust Backdoor Contamination Detection

A security threat to deep neural networks (DNN) is backdoor contamination, in which an adversary poisons the training data of a target model to inject a Trojan so that images carrying a specific trigger will always be classified into a specific label. Prior research on this problem assumes the dominance of the trigger in an image's representation, which causes any image with the trigger to be recognized as a member in the target class. Such a trigger also exhibits unique features in the representation space and can therefore be easily separated from legitimate images. Our research, however, shows that simple target contamination can cause the representation of an attack image to be less distinguishable from that of legitimate ones, thereby evading existing defenses against the backdoor infection. In our research, we show that such a contamination attack actually subtly changes the representation distribution for the target class, which can be captured by a statistic analysis. More specifically, we leverage an EM algorithm to decompose an image into its identity part (e.g., person, traffic sign) and variation part within a class (e.g., lighting, poses). Then we analyze the distribution in each class, identifying those more likely to be characterized by a mixture model resulted from adding attack samples to the legitimate image pool. Our research shows that this new technique effectively detects data contamination attacks, including the new one we propose, and is also robust against the evasion attempts made by a knowledgeable adversary.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	ccs-template.tex 

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

\subsection{Effectiveness}

\vspace{5pt}\noindent\textbf{Against TACT attacks}. 

\vspace{5pt}\noindent\textbf{False positive analysis}. 

\subsection{Robustness}

\vspace{5pt}\noindent\textbf{Whitebox attacks against SCANNER}. 

\vspace{5pt}\noindent\textbf{Transferability analysis}. 


\subsection{Robustness}


In this section, we demonstrates our experimental results about how to defeats current defences through Cover-Target, and the effectiveness of our defence against various attacks, on three image classification tasks.


\subsection{Experiment Setup}
\label{subsec:setup}

\begin{table*}[tbh]
  \centering
    \caption{Information about datasets and model architectures.}
	\begin{tabular}{|c|c|c|c|c|c|}
	\hline
	  Dataset & \# of Classes & \# of Training Images & \# of Testing/Validation Images & Input Size & Model Architecture\\
    \hline
	GTSRB & 43 & 39,209 & 12,630 & 32 x 32 x 3& 6 Conv + 2 Dense \\
	\hline
	ILSVRC2012 & 1,001 & 1,281,167 & 49,984 & 300 x 300 x 3 & ResNet50 \\
	\hline
	MegaFace & 647,608 & 4,019,408 & 91,712 (FaceScrub) & 128 x 128 x 3 & ResNet101 \\
	\hline
	
	\end{tabular}
	
	\label{tb:datasets}
\end{table*}

\begin{figure}[ht]
	\centering
  \begin{subfigure}{0.11\textwidth}
		\includegraphics[width=\textwidth]{figure/normal_lu.png}
		\caption{}
  \end{subfigure}
  \begin{subfigure}{0.11\textwidth}
		\includegraphics[width=\textwidth]{figure/normal_md.png}
		\caption{}
  \end{subfigure}
  \begin{subfigure}{0.11\textwidth}
		\includegraphics[width=\textwidth]{figure/uniform.png}
		\caption{}
  \end{subfigure}
  \begin{subfigure}{0.11\textwidth}
		\includegraphics[width=\textwidth]{figure/solid_rd.png}
		\caption{}
		\label{trigger:solid_rd}
  \end{subfigure}
 
	\caption{Four triggers. (a) A normal distribution centered on the top-left of the image. (b) A normal distribution centered on the middle of the image. (c) A uniform distribution covering all the image. (d) A white-box on the down-right of the image.  }
	\label{fig:triggers}

\end{figure}

\begin{table*}[tbh]
\centering
\caption{Models' Top-1 Accuracy and Success Rate of Attack.}
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{3}{c|}{Top-1 Accuracy}              & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Success Rate of Attack of\\ Poisoned Model\end{tabular}} \\ \cline{2-4}
                         & Pre-trained Model & Clean Model & Poisoned Model &                                                                                                     \\ \hline
GTSRB                    &       93.6\%     &    96.4\%  &    95.2\%        &        88.5\%                                                                                             \\ \hline
ILSVRC2012               &        72.9\%    &     76\%    &                &                                                                                                     \\ \hline
MegaFace                 &      66.7\%      &    71.4\%  &    70.6\%       &                                                                                                     \\ \hline
\end{tabular}
\label{tb:att_perf}
\end{table*}


Our experiments built on three tasks: (1) Traffic Sign Recognition. (2) Object Classification. (3) Face Recognition. Details of each task and associated dataset are described below. A brief summary is also included in Table~\ref{tb:datasets}. For brevity, we left the detailed description of training parameters and model architectures in Appendix~\ref{app:train}.

\vspace{3pt}\noindent$\bullet$\textit{ Traffic Sign Recognition (GTSRB)}.  This task is to  recognize different traffic signs in the self-driving scenario. For solving this task, we trained our backbone model with a simple architecture of 6 convolution layers and 2 dense layers (Table~\ref{tb:gtsrb}) on the German Traffic Sign Benchmark (GTSRB) dataset which contains 39.2K training images and 12.6K testing images of 43 different signs~\cite{Stallkamp2012}.  

\vspace{3pt}\noindent$\bullet$\textit{ Object Classification (ILSVRC2012)}.  This task is to  recognize general objects from images. A well-known dataset, Large Scale Visual Recognition Challenge 2012 (ILSVRC2012)~\cite{ILSVRC15}, was used to train our backbone model ResNet50~\cite{he2016deep}. This dataset contains 1.2M images from 1001 categories.

\vspace{3pt}\noindent$\bullet$\textit{ Face Recognition (MegaFace)}.  This task is to  recognize human face. We used one of the biggest datasets, MegaFace~\cite{nech2017level} containing 4M images of 647K identities, to train our backbone model ResNet101~\cite{he2016deep}. And, specifically, as guided by description on~\cite{MegaFace88:online}, we test our model on FaceScrub~\cite{ng2014data} and distracted by other 1M distractor images~\cite{MegaFace41:online}.

\noindent\textbf{Attack Configuration}. Guided by our adversarial model (Section~\ref{subsec:adversarial_model}), for each dataset, we first train a model on a hold-on dataset containing three quarters of the total training images, and fine-tune this pre-trinaed model on the rest data that may be poisoned by attackers. Those infected images generated by stamping a trigger to clean images and labelled by a chosen target label, which follows the approach proposed by Chen et al.~\cite{chen2017targeted}. The number of injected images varies from case to case and will be investigated in~\ref{subset:num_poison_inputs}. The trigger is selected from four kinds of patterns demonstrated on Fig~\ref{fig:triggers} and scaled to as the same as the input size of each task. And there are may multiple target labels and will be assigned before the fine-tuning.

To measure the performance of backdoor attacks, we calculate the top-1 accuracy on the testing set for each model, as well as the success rate of attack. The success rate of attack measures the percentage of images stamped by the trigger and classified into the target label. As a benchmark, we also calculate the top-1 accuracy of the clean models that is fine-tuned on clean images. These performances are reported in Table~\ref{tb:att_perf}. All poisoned models achieve high success rate of attack and maintain low impact on the top-1 accuracy, compared with the clean one. To be noticed that all the poisoned models have higher top-1 accuracy than their pre-trained model, demonstrating the stealthiness of poison attack.     

\subsection{Failure of Current Defences}
\label{subsec:current_defences}
In this section, we discuss the ineffectiveness of previous four defences. Without special explanation, we only use the white-box trigger (Fig~\ref{trigger:solid_rd}) to launch our attack.

\noindent\textbf{Neural Cleanse (NC).}
We rebuilt the Neural Cleanse~\cite{wangneural2019} defence, and our code published on~\cite{TDteachb82:online}. Specifically, Neural Cleanse tries to find a global backdoor trigger for each class and then recognize such classes with small trigger (in L1 norm) as infected class. We found global backdoor trigger by adding a mask layer $A(\cdot)$ right behind the input layer of our models. If the input image is $x$, then
\begin{equation}
\begin{array}{c@{\quad}l}
A(x) &= (1-\kappa)\cdot x + \kappa \cdot \delta \\
\kappa &= (\tanh(W_{\kappa})+1)/2 \\
\delta &= \tanh(W_{\delta})
\end{array}
\end{equation}
where $\kappa$ is the trigger mask and $\delta$ is the trigger pattern. We constrain their values be in the feasible range through $\tanh(\cdot)$ function. Putting together, for a fixed model $F(\cdot)$, we optimize the following function to find the global trigger for class $t$:

\begin{equation}
\begin{array}{c@{\quad}l}
\min_{W_{\kappa}, W_{\delta}} & \sum_{x \in \mathcal{X}} l(y_t, F(A(x))) + \lambda \cdot |\kappa|  \\
\end{array}
\end{equation}
where $y_t$ is the ground truth of class $t$, $l(\cdot)$ is the loss function of the classification and $\lambda$ is the weight of the L1 norm of the mask. Following~\cite{wangneural2019}, we set $\lambda$ correspondingly and ensure > 95\% of clean images can be successfully misclassfied (Table~\ref{tb:lambda}).

\begin{table}[tbh]
\centering
\caption{Lambda choosing and their percentage of misclassification.}
\begin{tabular}{|c|c|c|}
\hline
Dataset    & $\lambda$ & \begin{tabular}[c]{@{}c@{}}Percentage of Clean Images \\ Stamped by Trigger and Misclassfied \\ (with one time of std)\end{tabular} \\ \hline
GTSRB      & 0.1       & 96\% $\pm$ 0.7\%                                                                       \\ \hline
ILSVRC2012 & 1         &                                                                                   \\ \hline
MegaFace   & 1         &                                                                                   \\ \hline
\end{tabular}
\label{tb:lambda}
\end{table}

Our reproduction works well when defend against~\cite{chen2017targeted}. Fig~\ref{fig:norm_NC} shows the norm of global backdoor triggers for each class. Apparently, the norm of those infected class is far way from those norms for intact labels.

However, it is defeated by Cover-Target attack. Specifically, for each task, we chose one source label and two other labels as covering. 

Fig~\ref{fig:norm_NC} also demonstrate the results of Neural Cleanse facing Cover-Target attack. We observed that the norm of infected labels is totally mixed with those of intact labels, further, showing that Neural Cleanse can not detect out these infected labels.


\noindent\textbf{STRIP.}
STRIP~\cite{STRIP} tried to detect whether a input image is infected by blending it with images from other classes and checking that whether the blended images has low entropy. If it is, then the input image is clean, otherwise the image has been infected. 

The blending process can be expressed as:
\begin{equation}
\begin{array}{c@{\quad}l}
x_{blend} = \alpha x_{test} + (1-\alpha) x_{others}
\end{array}
\end{equation}
where $x_{blend}$ is the blended image we got, $x_{test}$ is the currently testing image and $x_{others}$ is the image from other classes.
We tested STRIP by setting $\alpha = 0.5$, i.e., taking the average of these two inputs. Our test was built on GTSRB dataset. Specifically, we launched the Cover-Target attack with settings: 0 is the target label, 1 is the source label and 11 & 12 are the cover labels, to get the backdoored model. Then, we used this model to generate logits for blended inputs: infected inputs blended with intact inputs, intact inputs blended with other intact inputs.

Fig~\ref{fig:entropy_STRIP} compares entropy of those two kinds of logits. To be noticed that, guided by STRIP paper, we normalized the entropy by subtracting the minimum entropy and then dividing the results by the difference between the minimum entropy and the maximum entropy. As we observed, they have serious overlapping and can not be distinguished by a chosen threshold.
\begin{figure}[ht]
	\centering
  \begin{subfigure}{0.23\textwidth}
		\includegraphics[width=\textwidth]{figure/entropy_strip.eps}
		\subcaption{}
		\label{fig:entropy_STRIP}
  \end{subfigure}
  \begin{subfigure}{0.245\textwidth}
		\includegraphics[width=\textwidth]{figure/alpha_strip.eps}
		\subcaption{}
		\label{fig:alpha_STRIP}
  \end{subfigure}
 
	\caption{Entropy of STRIP defence on GTSRB. (a) shows the normalized entropy. (b) shows the original entropy with one time of the standard deviation.}

\end{figure}

Further, we also investigated the impact of the blending ratio $\alpha$. Fig~\ref{fig:alpha_STRIP} shows the original entropy (without normalization) and teaches us that no matter which $\alpha$ is chosen STRIP can not defeat the Cover-Target attack. We discuss that, it is because Cover-Target attack binds the trigger with the between-class feature. When the between-class feature becomes ambiguous by blending, the affect of the trigger also goes vague and will not induce misclassification.

\noindent\textbf{SentiNet.} SentiNet~\cite{sentinet} used a different way to detect the infected input. When a input comes, SentiNet split the input into two parts, classification-matter part and the rest. Then, authors pasted classification-matter part onto other clean images (hold-on set) and found out the classification results of these overlaid images, at the meantime, they also investigated the effect of the rest part to the results. In authors' view, for an infected input, pasting its matter region onto clean images will result in misclassification of this overlaid image, while the rest part will not affect the results, i.e., the image pasted on the rest part still has high confidence on its original class.

In SentiNet, splitting is challenge and may fail. Thus we tested this defence in a simple manner on MegaFace. Specifically, we regarded the trigger pattern area as the classification-matter part for infected images, the centre area as the matter part for intact images. That is because we have already aligned facial images and held that the face is always at the center of the image. Following author's method, we represent every image as a point in the two-dimensional space. The y-axis represents the fooled count $Fooled$, i.e., the $Fooled$ plus $1$, if misclassification after pasting the matter part, and is divided by the total number at the end. The x-axis represents the average confidence $AvgConf$ of the decision after pasting the rest part. 

Empirically, the infected input will stay on the top-right corner of the figure. Fig~\ref{fig:plots_sentinet} demonstrates our results. We observe that, under Cover-Traget attack, infected images stay on the down-right corner and are mixed with those intact images. This demonstrates the powerless of SentiNet against our attack.

\begin{figure}[ht]
	\centering
  \begin{subfigure}{0.45\textwidth}
		\includegraphics[width=\textwidth]{figure/plots_sentinet.eps}
  \end{subfigure}
  
 
	\caption{Entropy of STRIP defence on GTSRB. (a) shows the normalized entropy. (b) shows the original entropy with one time of the standard deviation.}
	\label{fig:plots_sentinet}

\end{figure}

\noindent\textbf{Activation Clustering (AC).} AC~\cite{ac_attack} proposed that infected images will result in different activations of model from intact images. Here we argue that this different will become vague when dealing with Cover-Target attack, as in this attack the feature of benign and the feature of trigger are tightly connected. Only the trigger will not lead to backdoor. Thus k-mean used by AC will loss its effectiveness, especially for complex task (face recognition).

We launched a Cover-Target attack on GTSRB with settings: 0 is the target label and 1 is the source label and 11 & 12 are the cover labels. Then we used 2-means to cluster the activations. 
Fig~\ref{fig:score_ac} illustrates the sihouette scores, the criteria used by AC to measure how well 2-means fit the data and decide which class is infected. We observe that, there is no clean cut between the infected class and intact classes. Specifically, we saw a lot of outliers lay outside the label 0' box (0 is the target label), representing 2-means can not fit this class well. This conclusion is clearly different from the requirement of being an infected class in AC, which confirms that AC will defeated by Cover-Target attack. 

\begin{figure*}[ht]
	\centering
  \begin{subfigure}{\textwidth}
		\includegraphics[width=\textwidth]{figure/score_ac.eps}
  \end{subfigure}
 
	\caption{Sihouettte scores of AC defence on GTSRB dataset. 0 is the target label (infected class), 1 is the source label and others are intact labels. Box plot shows quartiles.}
	\label{fig:score_ac}

\end{figure*}

\subsection{Effectiveness of Our Defence}
\label{subsec:effectiveness}

In this section, we demonstrate the effectiveness of our method defending against Cover-Target attack with various triggers.

Fig~\ref{fig:effect_4triggers_3tasks} shows the distribution of our judging criterion $\tilde{J}$ for four triggers and three tasks. Each row is represents a task and each column represents a trigger. For brevity, we kept $0$ as the target label in these twelve experiments. From figures, we observe that $\tilde{J}_0=1$ for all the cases and $\tilde{J}$ for other labels are almost $0$. That is to say $0.5$ as we set in Section~\ref{subsec:approach} is very loose and robust against various cases.

Above results prove that, in one backdoor injection scenario, our defence is very effective for Cover-Target attack that beats almost current defences. Next we talk about advanced cases.


\subsection{Robustness against Advanced Backdoors}
\label{subsec:robustbess}
Guided by~\cite{wangneural2019} where authors lists five types of advanced backdoor attacks, we discuss two of them in this section. 
The rest three types attacks actually have been covered in Section~\ref{subsec:effectivness} where our defense works well on them.

\vspace{3pt}\noindent$\bullet$\textit{Multiple Infected Labels with Separate Triggers}

In this experiment, for $n$ triggers case, we set $(i-1)$ as the target label for the $i^{th}$ trigger. Fig~\ref{fig:mvm} demonstrates results of different $n$. We observe that when the $n$ increase, our defence performance drop. We discuss that this is because the global model we built is affected by the infected data.

There is a very easy mitigation method. We build the global model just on the predictions of hold-on data. Fig~\ref{fig:mit_mvm} shows that this mitigation works perfect. While this mitigation requires big enough hold-on dataset which is one limitation of our defence. 


\vspace{3pt}\noindent$\bullet$\textit{Single Infected Label with Multiple Triggers}

As usual, we set 0 as the target label, and try to inject multiple triggers for label 0. As shown in Fig~\ref{fig:ovm}, when the number of triggers increase, $\tilde{J}_0$ varies and the classification performance decrease. And once more than 8 triggers have been injected the classification performance drop significantly. This will break the stealthiness of attack.

Actually, in the view of our defence, this more-in-one attack is no different between normal cases, compact multiple classes into one class. Thus our defence works well as usual.



